Poncelet Triangles: a Theory for Locus Ellipticity

We present a theory which predicts if the locus of a triangle center over certain Poncelet triangle families is a conic or not. We consider families interscribed in (i) the confocal pair and (ii) an outer ellipse and an inner concentric circular caustic. Previously, determining if a locus was a conic was done on a case-by-case basis. In the confocal case, we also derive conditions under which a locus degenerates to a segment or a circle. We show the locus' turning number is +/- 3, while predicting its monotonicity with respect to the motion of a vertex of the triangle family.

==> 000_edits.tex <==
Referee's report on BZAG-D-21-00166

HARD: 

- shorten proof parts
- make paper two pages shorter

EASY:

- first sentence of abstract: altered as suggested
- removed "locus" and "affine" from keywords
- Changed style ``[ref]'' to ``found in [ref]''.
- Page 1: Figure 1 in the right position 
- Figure 2: though reviewer asked to remove it, it contains some important info referred to in Appendix A. We would like to keep it but with a rearrangement it now only occupies 1/2 of the original size.
- If figure 2 can be kept, we don't need to reformulate the first three lines of page 3.
- Page 2, line -3: "we show" ---> "We show"
- Page 3, At the end of "Main results" reference the following surveys:
- Added paragraph to the end of "Main results" to the effect that the derived results aren't found in well-known surveys of Poncelet's theorem. 

- Page 4, line -2: "over the complex the 
unit circle," was changed to
''as $\lambda$ sweeps the unit circle monotonically''
%"3 cycles of $\lambda$ (from 0 to $6\pi$)
- Page 5, line 1: deleted "also" before "proved"
- Appendix A was removed (as it only contained one table). The table was reinserted near its first reference in the text (Section 4).
-  Changed title of Appendix B (now Appendix A) to "Triangle centers whose locus is an ellipse"
- demoted section 6 to a subsection at the end of section 5.
- to save space, removed the rather short table of symbols.
- fixed reference [9]: "Poncelet" (capital "P") 
- corrected Depp et al. reference, in accordance with Math reviews
- Table 1 was "transposed" and now occupies 1/2 of the height of the original.
- cropped figure 4 significantly (only locus of X20 is not shown in its entirety)



==> 000_refcheck.tex <==
\usepackage{refcheck}
% make refcheck work w cref
% https://tex.stackexchange.com/questions/87610/making-refcheck-work-with-cleveref
\makeatletter
\newcommand{\refcheckize}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[1]{%
    \csname @@\string#1\endcsname{##1}\@for\@temp:=##1\do{\wrtusdrf{\@temp}\wrtusdrf{{\@temp}}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\newcommand{\refcheckizetwo}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[2]{%
    \csname @@\string#1\endcsname{##1}{##2}\wrtusdrf{##1}\wrtusdrf{{##1}}\wrtusdrf{##2}\wrtusdrf{{##2}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\makeatother

\refcheckize{\cref}
\refcheckize{\Cref}
\refcheckizetwo{\crefrange}
\refcheckizetwo{\Crefrange}

==> 240_app_elliptic_axes.tex <==
\subsection{Confocal}

\noindent As above, $\delta=\sqrt{a^4-a^2b^2+b^4}$. Also, the following explicit expressions were given for the semi-axes of the $N=3$ caustic \cite{garcia2019-incenter}:

\begin{equation*}
a_c=\frac{a\left(\delta-{b}^{2}\right)}{c^2},\;\;\;
b_c=\frac{b\left({a}^{2}-\delta\right)}{c^2}\cdot
\end{equation*}

Two concentric, axis-aligned ellipses can generate a Poncelet triangle family if and only if $a/a_c+b/b_c=1$ \cite{griffiths1978}, which holds above.

\subsection{\torp{$X_1$}{X1} and Excenters}
 
\begin{equation*}
 a_1=\frac{\delta-{b}^{2}}{a},\;\;\;
 b_1=\frac{{a}^{2}-\delta}{b}
\end{equation*}
 
The locus of the Excenters is an ellipse with semi-axes:
 
\begin{equation*}
 a_e=\frac{{b}^{2}+\delta}{a},\;\;\; 
 b_e=\frac{{a}^{2}+\delta}{b}
\end{equation*}
 
\noindent Notice it is similar to the $X_1$ locus, i.e., $a_1/b_1=b_e/a_e$. 

% razao do bilhar pela interna 
%\begin{align*}
%    a_eb_e-a_1b_1=&\frac{2(a^4+b^4)}{ab}\\  
%\frac{a_1b_1}{\frac{r}{R}}=& \frac{a^2-b^2}{2ab}= \frac{c^2}{2ab}\end{align*}
%The ratio of their areas *** ronaldo, related to $r/R$.

\subsection{\torp{$X_2$}{X2} (similar to billiard)}

\begin{equation*}
 \left(a_2,b_2\right)=k_2\left(a,b\right),\;\textrm{where}\; k_2=\frac{2\delta -{a}^{2}-{b}^{2}}{3c^2}
\end{equation*}

 \subsection{\torp{$X_3$}{X3} (similar to rotated caustic)}
 
\begin{equation*}
 a_3=\frac{{a}^{2}-\delta}{2a},\;\;\;
 b_3=\frac{\delta-{b}^{2}}{2b}
\end{equation*}

Additionally, when $a/b= \frac{\sqrt{2\sqrt{33}+2}}{2} \;{\simeq}\;1.836$, $b_3=b$, i.e., the top and bottom vertices of the locus of $X_3$ coincide with the billiard's.

\subsection{\torp{$X_4$}{X4} (similar to rotated billiard)}
\label{app:x4}
 
\begin{equation*}
\scriptsize
\left(a_4,b_4\right)=\left(\frac{k_4}{a},\frac{k_4}{b}\right),\;  k_4=\frac{  ({a}^{2}+{b}^{2})\delta-2\,{a}^{2}{b}^{2} }{c^2}
% a_4={\frac{ \left( {a}^{2}+{b}^{2} \right) \delta-2\,{b}^{2}{a}^{2}}{\left({a}^{2}-{b}^{2}\right)a}},\;\;\;
% b_4={\frac{ \left( {a}^{2}+{b}^{2} \right) \delta-2\,{b}^{2}{a}^{2}}{\left({a}^{2}-{b}^{2}\right)b}}
\end{equation*}

Additionally:
\begin{itemize}
\item When
$a/b=a_4=\sqrt{2\,\sqrt {2}-1}\;{\simeq}\;1.352$, $b_4=b$, i.e., the top and bottom vertices of the locus of $X_4$ coincide with the billiard top and bottom vertices.

%Figure~\ref{fig:orthocenter_loci}b.

\item Let $a_4^*$ be the positive root of
${x}^{6}+{x}^{4}-4\,{x}^{3}-{x}^{2}-1=0$, i.e.,
$a_4^{*}={\simeq}\;1.51$. When $a/b=a_4^{*}$, $a_4=b$ and $b_4=a$, i.e., the locus of $X_4$ is identical to a rotated copy of billiard. %Figure~\ref{fig:orthocenter_loci}c. 
\end{itemize}

\subsection{\torp{$X_5$}{X5}}

%\begin{align*}
% a_5=&   \frac{-{a}^{2} \left( {a}^{2}+3\,{b}^{2} %\right) +\delta \left( 3\,{a}^{2}+{b}^{2} \right) }{4a \left( {a}^{2}-{b}^{2} \right) }\\
%  b_5=&{\frac{-{b}^{2} \left( 3\,{a}^{2}+{b}^{2} %\right) +\delta \left( {a}^{2}+3\,{b}^{2} \right) }{4b\left( {a}^{2}-{b}^{2}\right) }}
%\end{align*}
   			%
\begin{equation*}
  a_5=\frac{- w'_5(a,b)+ w''_5(a,b) \delta}{ w_5(a,b)},\;\;\;b_5=\frac{ w'_5(b,a)-{w''_5(b,a) \delta}}{w_5(b,a)}
\end{equation*}
 
\begin{equation*}
 w'_5(u,v)=u^2(u^2+3v^2),\;\;\;w''_5(u,v)=3u^2+ v^2,\;\;\;w_5(u,v)=4u(u^2-v^2).
\end{equation*}

\subsection{\torp{$X_7$}{X7} (similar to billiard)}
    
\begin{equation*}
\left(a_7,b_7\right)=k_7\left(a,b\right),\;\;  k_7=\frac{2\delta - {a}^{2}-{b}^{2}}{c^2}
%   a_7= \frac{\left(2\delta - {a}^{2}-{b}^{2} \right) a}{{a}^{2}-{b}^{2}},\;\;
%   b_7= \frac{ \left(2\delta - {a}^{2}-{b}^{2}\right) b}{{a}^{2}-{b}^{2}}
\end{equation*}

\subsection{\torp{$X_8$}{X8}}

\begin{equation*}
 a_{8}= {\frac{ ({b}^2-\delta)^2 }{a c^2   }},\;\;\;
 b_{8}={\frac{  ({a}^{2} -\delta )^2  }{b c^2 }}
\end{equation*}

\subsection{\torp{$X_{10}$} (similar to rotated billiard)}

\begin{equation*}
\left(a_{10},b_{10}\right)=\left(\frac{k_{10}}{a},\frac{k_{10}}{b}\right),\;\;   k_{10}=\frac{ \left( {a}^{2}+{b}^{2} \right)\delta-{a}^{4}-{b}^{4}}{2 c^2}
%a_{10}={\frac{ \left( {a}^{2}+{b}^{2} \right) \delta-{a}^{4}-{b}^{4}}{ 2\left( {a}^{2}-{b}^{2} \right) a}}, \;\;\;
%b_{10}={\frac{ \left( {a}^{2}+{b}^{2} \right) \delta-{a}^{4}-{b}^{4}}{ 2\left( {a}^{2}-{b}^{2} \right) b}}
\end{equation*}

\subsection{\torp{$X_{11}$}{X11} (identical to caustic)}
 
\begin{equation*}
    a_{11}=a_c,\;\;\;b_{11}=b_c
\end{equation*}

\subsection{\torp{$X_{12}$}{X12}}
\begin{equation*}
    a_{12}=\frac{ - w'_{12} (a,b)+ w''_{12}(a,b) \delta}{ w_{12} (a,b)},\;\;\;b_{12}=\frac{   w'_{12}(b,a)-w''_{12}(b,a)\delta}{ w_{12}(b,a)}
\end{equation*}

\begin{align*}
w'_{12}(u,v)=&
		  v^2(15\,{u}^{6}+12\,{v}^{2}{u}^{4}+3\,{u}^{2}{v}^{4}+2\,{v}^{6})\\
w''_{12}(u,v)= & 7\,{u}^{6}+12\,{v}^{2}{u}^{4}+11\,{u}^{2}{v}^{4}+2\,{v}^{6}  \\
w_{12}(u,v)=&  u( 7\,{u}^{6}+11\,{v}^{2}{u}^{4}-11\,{u}^{2}{v}^{4}-7\,{v}^{6}).
%
%b_{12}=&  {\frac{- \,{a}^{2}(2a^6+3\,{b}^{2}{a}^{4}+12\,{a}^{2}{b}^{4}+15\,{b}^{6})+ \left( 2\,{a}^{6}+11\,{b}^{2}{a}^{4}+12\,{a}^{2}{b}^{4}+7\,{b}^
	%	{6} \right) \delta}{b \left( 7\,{a}^{6
%		}+11\,{b}^{2}{a}^{4}-11\,{a}^{2}{b}^{4}-7\,{b}^{6} \right) }}
\end{align*} 
 
\subsection{\torp{$X_{20}$}{X20}}

\begin{equation*}
a_{20}=     {\frac{{a}^{2} \left(3b^2- {a}^{2}  \right) -2b^2\,\delta }{ ac^2}}, \;\;\;
b_{20}=   {\frac{{b}^{2} \left(  {b}^{2} -3a^2\right) +2a^2\,\delta}{b c^2 }}
\end{equation*}

\subsection{\torp{$X_{21}$}{X21}}

 %\begin{align*}
% a_{21}=&     {\frac{-{a}^{4}-{a}^{2}{b}^{2}-2\,{b}^{4}+2\, \left( {a}^{2}+{b}^{2}
 %	\right) \delta}{a \left( 3\,{a}^{2}+5
 %		\,{b}^{2} \right) }}\\
 %b_{21}=&  {\frac{2\,{a}^{4}+{a}^{2}{b}^{2}+{b}^{4}-2\, \left( {a}^{2}+{b}^{2}
 %		\right) \delta}{b  }}
 %\end{align*}

\begin{equation*}
    a_{21}=\frac{-w'_{21}(a,b)+ w''_{21}(a,b) \delta}{ w_{21}(a,b)},\;\;\;b_{21}=\frac{ w'_{21}(b,a)- \,  w''_{21}(b,a)\delta}{ w_{21}(b,a)}\\
\end{equation*}
{\small  
\begin{equation*}
w'_{21}(u,v)={u}^{4}+{u}^{2}{v}^{2}+ \,{v}^{4},\;\;w''_{21}(u,v)= 2( {u}^{2}+{v}^{2}),\;\;w_{21}(u,v)=u\left( 3\,{u}^{2}+5\,{v}^{2} \right)
\end{equation*}
}
\subsection{\torp{$X_{35}$}{X35}}

%\begin{align*}
%a_{35}=&     {\frac{ \left( 7\,{a}^{2}+{b}^{2} \right)  \left( {a}^{2}+{b}^{2}
	%\right) \delta-{b}^{2} \left( 11\,{a}
%		^{4}+4\,{a}^{2}{b}^{2}+{b}^{4} \right) }{a \left( 7\,{a}^{4}+18\,{a}^{
%			2}{b}^{2}+7\,{b}^{4} \right) }} \\
%b_{35}=&  {\frac{ \left( {a}^{2}+7\,{b}^{2} \right)  \left( {a}^{2}+{b}^{2}
%		\right) \delta-{a}^{2} \left( {a}^{4}
%		+4\,{a}^{2}{b}^{2}+11\,{b}^{4} \right) }{b \left( 7\,{a}^{4}+18\,{a}^{
	%		2}{b}^{2}+7\,{b}^{4} \right) }}
%\end{align*}

\begin{align*}
a_{35}=&\frac{-w'_{35}(a,b)+w''_{35}(a,b) \delta}{w_{35}(a,b)},\;\;\;b_{35}=\frac{-w'_{35}(b,a)+w''_{35}(b,a)\delta}{w_{35}(b,a)} \\
w'_{35}(u,v)=&v^2( 11\,{u}^{4}+4\,{u}^{2}{v}^{2}+{v}^{4} ),\;\;\;w''_{35}(u,v)=\left( 7\,{u}^{2}+{v}^{2} \right)  \left( {u}^{2}+{v}^{2}\right)\\
w_{35}(u,v)=& u(7\,{u}^{4}+18\,{u}^{2}{v}^{2}+7\,{v}^{4} )
\end{align*}

\subsection{\torp{$X_{36}$}{X36}}
%\begin{equation*}
%a_{36}= \,{\frac{ \left( %3\,{a}^{2}-{b}^{2} \right) %\delta+{b}^{2} \left( {a}^{2}+{b}^{2} %\right) }{3a \left( a^2-b^2 \right)}}, \;\;\;
%b_{36}=  {\frac{ \left( %{a}^{2}-3\,{b}^{2} \right) %\delta+{a}^{2} \left( {a}^{2}+{b}^{2} %\right) }{3b(  \,{a}^{2} - \,{b
%		}^{2})}}
%\end{equation*}

\begin{equation*}
    a_{36}=\frac{w'_{36}(a,b)+ w''_{36}(a,b)\delta }{w_{36}(a,b)},\;\;\;b_{36}=\frac{  -w'_{36}(b,a)  -w''_{36}(b,a)\delta}{w(b,a)}
\end{equation*}

\begin{equation*}
w'_{36}(u,v)=	{v}^{2} \left( {u}^{2}+{v}^{2} \right),\;\;\;w''_{36}(u,v)=  3\,{u}^{2}-{v}^{2},\;\;\;
w_{36}(u,v)=3u \left(u^2-v^2\right)
\end{equation*}

\subsection{\torp{$X_{40}$}{X40} (similar to rotated billiard)}
\label{app:x40}
%ron conferido
\begin{equation*}
a_{40}=\frac{ c^2}{a},\;\;\;
b_{40}=\frac{ c^2}{b}
\end{equation*}
Additionally:
\begin{itemize}
\item When $a/b= \sqrt{2}$, $b_{40}=b$, i.e., the top and bottom vertices of the $X_{40}$ locus coincides with the billiard's.

\item When $a/b=(1+\sqrt{5})/2=\phi\;{\simeq}\;1.618$, $b_{40}=a$ and $a_{40}=b$, i.e., the $X_{40}$ locus is identical to a rotated copy of billiard.
\end{itemize}
%*** ronaldo: $a/b$ where $X_40$ touches top and bottom %of billiard, and is identical to billiard.

\subsection{\torp{$X_{46}$}{X46}}
      
 %\begin{align*}
 %a_{46}=&             {\frac{ \left( {a}^{2}-{b}^{2} \right)  \left(  \left( 5\,{a}^{2}+{b}^{2} \right) \delta+{b}^{2} \left(3\,
   % 	{a}^{2}-{b}^{2} \right)  \right) }{a \left( 5\,{a}^{4}-6\,{a}^{2}{b}^{
    %			2}+5\,{b}^{4} \right) }} \\
 %b_{46}=&  -{\frac{ \left( {a}^{2} \left( {a}^{2}-3\,{b}^{2} \right) -\delta \left( {a}^{2}+5\,{b}^{2} \right) 
   %  		\right)  \left( {a}^{2}-{b}^{2} \right) }{b \left( 5\,{a}^{4}-6\,{a}^
    %		{2}{b}^{2}+5\,{b}^{4} \right) }}
% \end{align*}

\begin{equation*}
    a_{46}=\frac{w'_{46}(a,b)+w''_{46}(a,b) \delta}{ w_{46}(a,b) },\;\;\;b_{46}=\frac{-w'_{46}(b,a) - w''_{46}(b,a)\delta}{ w_{46}(b,a) }
\end{equation*}

\begin{align*}
w'_{46}(u,v)=& v^2(3\,{u}^{2}-{v}^{2} )(u^2-v^2),\;\;\;w''_{46}(u,v)= (5\,{u}^{2}+{v}^{2})(u^2-v^2) \\
w_{46}(u,v)=& v(5\,{u}^{4}-6\,{u}^{2}{v}^{2}+5\,{v}^{4} )
\end{align*}

\subsection{\torp{$X_{55}$}{X55} (similar to caustic)}
      
\begin{equation*}
a_{55}= {\frac{a\left(\delta-{b}^{2}
      		\right)}{{a}^{2}+{b}^{2}}},\;\;
       b_{55} =  { \frac{b \left( {a}^{2}-\delta
       	\right)}{{a}^{2}+{b}^{2}}}    
\end{equation*}    

\subsection{\torp{$X_{56}$}{X56}}
     
%\begin{align*}
%a_{56}=&  {\frac{-{b}^{2} \left( {a}^{4}-{a}^{2}{b}^{2}+2\,{b}^{4} \right) +
    %  		\left( 5\,{a}^{4}-5\,{a}^{2}{b}^{2}+2\,{b}^{4} \right)\delta}{a \left( 5\,{a}^{4}-6\,{a}^{2}{b}^{2}+5\,{b}
   %   		^{4} \right) }}  \\
%b_{56}=&  -{\frac{-{a}^{2} \left( 2\,{a}^{4}-{a}^{2}{b}^{2}+{b}^{4} \right) +
   %   		\left(2\,{a}^{4}-5\,{a}^{2}{b}^{2}+5\,{b}^{4} \right) \delta}{b \left( 5\,{a}^{4}-6\,{a}^{2}{b}^{2}+5\,{b}
      %		^{4} \right) }}
%\end{align*}
\begin{equation*}
a_{56}=  \frac{-w'_{56}(a,b) + w''_{56}(a,b) \delta}{  w_{56}(a,b) },\;\;\;   
b_{56}= \frac{ w'_{56}(b,a) - w''_{56}(b,a) \delta}{  w_{56}(b,a) } 
\end{equation*}

\begin{align*}
w'_{56}(u,v)=&v^2( {u}^{4}-{u}^{2}{v}^{2}+2\,{v}^{4}),\;\;\;w''_{56}(u,v)= 5\,{u}^{4}-5\,{u}^{2}{v}^{2}+2\,{v}^{4}  \\
w_{56}(u,v)=&u(5\,{u}^{4}-6\,{u}^{2}{v}^{2}+5\,{v}^{4} ) 
\end{align*}

\subsection{\torp{$X_{57}$}{X57} (similar to billiard)}
\begin{equation*}
\left(a_{57},b_{57}\right)=k_{57}\left(a,b\right),\;\;   k_{57}=\frac{c^2}{\delta}
%a_{57}=\frac{a (a^2- b^2)}{ \delta}, \;\;\;
%b_{57}=\frac{b (a^2- b^2)}{ \delta}
\end{equation*}

\subsection{\torp{$X_{63}$}{X63} (similar to billiard)}
\begin{equation*}
\left(a_{63},b_{63}\right)=k_{63}\left(a,b\right),\;\; k_{63}=\frac{c^2}{a^2+b^2}
%a_{63}={\frac{a \left( {a}^{2}-{b}^{2} \right) }{{a}^{2}+{b}^{2}}},\;\;\;
%b_{63}= {\frac{b \left( {a}^{2}-{b}^{2} \right) }{{a}^{2}+{b}^{2}}}
\end{equation*}

\subsection{\torp{$X_{65}$}{X65}}

%\begin{align*}
%a_{ 65}=&-{\frac{-{a}^{4}{b}^{2}-{a}^{2}{b}^{4}-2\,{b}^{6}- \left( {a}^{4}-3\,
%	{a}^{2}{b}^{2}-2\,{b}^{4} %\right) \delta}{a \left( a^2-b^2 \right)^{2}  }}\\
%b_{65}=&{\frac{-2\,{a}^{6}-{a}^{4}{b}^{2}-{a}^{2}{b}^{4}+ \left( 2\,{a}^{4}+3\,{b}^{2}{a}^{2}-{b}^{4}
 %    		\right)\delta}{b \left( {a}^{2}-{b}^{2} \right) ^{2}}}
%\end{align*}

\begin{align*}
a_{65}=& \frac{w'_{65}(a,b) + w''_{65}(a,b) \delta}{  w_{65}(a,b)},\;\;\;
b_{65}=\frac{-w'_{65}(b,a)- w''_{65}(b,a) \delta}{  w_{65}(b,a)}
\end{align*}

\begin{align*}
w'_{65}(u,v)=& {u}^{4}{v}^{2}+{u}^{2}{v}^{4}+2\,{v}^{6},\;\;\;
w''_{65}(u,v)={u}^{4}-3\,{u}^{2}{v}^{2}-2\,{v}^{4}\\
w_{65}(u,v)=&u\left( {u}^{2}-{v}^{2} \right) ^{2}
\end{align*}

\subsection{\torp{$X_{72}$}{X72}}
\begin{align*}
a_{72}=& \frac{w'_{72}(a,b) - w''_{72}(a,b) \delta }{w_{72}(a,b)},\;\;\;
b_{72}= \frac{-w'_{72}(b,a) + w''_{72}(b,a) \delta}{w_{72}(b,a) }
\end{align*}
{\small  
\begin{equation*}
w'_{72}(u,v)= {u}^{6}+2\,{u}^{2}{v}^{4}+{v}^{6},\;\;
w''_{72}(u,v)= (3\,{u}^{2}+{v}^{2}){v}^{2},\;\;
w_{72}(u,v)= u\left(u^2-v^2 \right)^{2}
\end{equation*}
}
%\begin{align*}
 %         a_{ 72}=&  {\frac{{a}^{6}+2\,{a}^{2}{b}^{4}+{b}^{6}
 %         -\delta {b}^{2} \left( 3\,{a}^{2}+{b}^{2} \right) }{a \left( a^2-b^2
  %        		\right) ^{2}  }} \\
%b_{72}=&  %{\frac{-{a}^{6}-2\,{a}^{4}{b}^{2}-{b}^{%6}+{a}^{2} \left( {a}^{2}+3\,{     	%		b}^{2} \right) \delta}{b \left( a^2-b^2
         %		\right) ^{2}  }}
%\end{align*}
          
\subsection{\torp{$X_{78}$}{X78}}
          
%\begin{align*}
%a_{78}=&  {\frac{5\,{a}^{6}-4\,{a}^{4}{b}^{2}+{a}^{2}{b}^{4}+2\,{b}^{6}-2\,
    %      		\delta{b}^{2} \left( {a}^{2}+{b}^{2}
      %    		\right) }{a \left( 5\,{a}^{4}-6\,{b}^{2}{a}^{2}+5\,{b}^{4} \right) }}  \\
%b_{78}=&  {\frac{-2\,{a}^{6}-{a}^{4}{b}^{2}+4\,{a}^{2}{b}^{4}-5\,{b}^{6}+2\,
  %        		\delta{a}^{2} \left( {a}^{2}+{b}^{2}
      %    		\right) }{b \left( 5\,{a}^{4}-6\,{b}^{2}{a}^{2}+5\,{b}^{4} \right) }}
%\end{align*} %%%%          
\begin{equation*}
a_{78}= \frac{w'_{78}(a,b) -w''_{78}(a,b) \delta }{w_{78}(a,b) },\;\;\;
b_{78}=  \frac{-w'_{78}(b,a)+w''_{78}(b,a) \delta}{w_{78}(b,a)} 
\end{equation*}

\begin{align*}
w'_{78}(u,v)=&5\,{u}^{6}-4\,{u}^{4}{v}^{2}+{u}^{2}{v}^{4}+2\,{v}^{6},\;\;\;w''_{78}(u,v)= 2\,{v}^{2} \left( {u}^{2}+{v}^{2}\right)\\
w_{78}(u,v)=&u \left( 5\,{u}^{4}-6\,{v}^{2}{u}^{2}+5\,{v}^{4} \right)\
\end{align*}

\subsection{\torp{$X_{79}$}{X79}}

%\begin{align*}
%a_{ 79}=&  {\frac{-{b}^{2} \left( 11\,{a}^{4}+4\,{b}^{2}{a}^{2}+{b}^{4} \right) + \left( 3\,{a}^{4}+12\,{b}^{2}{a}^{2}+{b}^{4} \right) \delta  }{a \left(a^2-b^2 \right)  \left( 3\,{a}^{2}+5\,{b}^{2} \right) }} \\
%b_{79}=&  {\frac{-{a}^{2} \left( {a}^{4}+4\,{b}^{2}{a}^{2}+11\,{b}^{4} \right) + \left( {a}^{4}+12\,{b}^{2}{a}^{2}+3\,{b}^{4}\right) \delta  }{b \left( a^2-b^2  \right)  \left( 5\,{a}^{2}+3\,{b}^{2} \right) }}
%\end{align*}

\begin{equation*}
a_{79}= \frac{-w'_{79}(a,b) + w''_{79}(a,b) \delta  }{w_{79}(a,b) }, \;\;\; 
b_{79}= \frac{  w'_{79}(b,a)- w''_{79}(b,a) \delta  }{  w_{79}(b,a)  }\end{equation*}

\begin{align*}
w'_{79}(u,v)=&{v}^{2}   11\,{u}^{4}+4\,{v}^{2}{u}^{2}+{v}^{4},\;\;\;w''_{79}(u,v)=& \left( 3\,{u}^{4}+12\,{u}^{2}{v}^{2}+{v}^{4} \right)   \\
w_{79}(u,v)=&u \left( u^2-v^2 \right) \left( 3\,{u}^{2}+5\,{v}^{2} \right)
\end{align*}

\subsection{\torp{$X_{80}$}{X80} }
      
\begin{equation*}
a_{80}={\frac{ \left( \delta-{b}^{2} 
      		\right)  \left( {a}^{2}+{b}^{2} \right)}{a c^2}},\;\;\;
b_{80}={\frac{ \left( {a}^{2}-\delta
      		\right)  \left( {a}^{2}+{b}^{2} \right)}{b c^2}}
\end{equation*}
      
\subsection{\torp{$X_{84}$}{X84} (similar to rotated caustic)}

\begin{equation*}
a_{84}=\frac{\left( {b}^{2}+\delta \right) c^2}{{a}^{3}},\;\;\;
b_{84}=\frac{\left( {a}^{2}+\delta \right) c^2}{{b}^{3}}
\end{equation*}
  
\subsection{\torp{$X_{88}$}{X88} (identical to billiard)}
      
\begin{equation*}
    a_{88}=a,\;\;\;b_{88}=b
\end{equation*}
      
\subsection{\torp{$X_{90}$}{X90}
}

%\begin{align*}
%a_{90}=& {\frac{ \left( {b}^{2} \left( 3\,{a}^{2}-{b}^{2} \right) + \left( {a} ^{2}+{b}^{2} \right) \delta \right) \left( {a}^{2}-{b}^{2} \right) }{a \left( {a}^{4}+2\,{b}^{2}{a}^{2}-7\,{b}^{4} \right) }} \\
%b_{90}=& -{\frac{ \left( -{a}^{2} \left( {a}^{2}-3\,{b}^{2} \right) + \left( {a}^{2}+{b}^{2} \right) \delta \right) \left( {a}^{2}-{b}^{2} \right) }{b \left( 7\,{a}^{4}-2\,{b}^{2}{a}^{2}-{b}^{4} \right) }}
%\end{align*}
\begin{equation*}
a_{90}= \frac{ w'_{90}(a,b) +  w''_{90}(a,b)\delta   }{w_{90}(a,b)},\;\;\;
b_{90}= \frac{w'_{90}(b,a)+w''_{90}(b,a) \delta  }{  w_{90}(b,a)}
\end{equation*}

\begin{align*}
w'_{90}(u,v)=&v^2(3u^2-v^2) (u^2-v^2),\;\;\;
w''_{90}(u,v)=u^4-v^4 \\
w_{90}(u,v)=& u \left( {u}^{4}+2\,{u}^{2}{v}^{2}-7\,{v}^{4} \right)
\end{align*}


\subsection{\torp{$X_{100}$ }{X100} (identical to billiard)}

\begin{equation*}
    a_{100}=a,\;\;\;b_{100}=b
\end{equation*}

%    \subsection{$X_{190}$ (identical to billiard)}
%\begin{equation*}
 %   a_{190}=a,\;\;\;b_{190}=b
%\end{equation*} 

\subsection{Homothetic}

\begin{align*}
	a_3=& \frac{a^2-b^2}{4a}, b_3=\frac{a^2-b^2}{4b}\\
	a_4=&\frac{a^2-b^2}{2a}, b_4=\frac{a^2-b^2}{2b}\\
	a_5=& \frac{a^2-b^2}{8a}, b_5=\frac{a^2-b^2}{8b} \\
	a_6=&\frac{a(a^2-b^2)}{2(a^2+b^2)}  ,b_6=\frac{b(a^2-b^2)}{2(a^2+b^2)} \\
	r_{13}=& \frac{a-b}{2}\\
	r_{14}=& \frac{a+b}{2}\\
	r_{15}=& \frac{(a-b)^2}{2(a+b)}\\
	r_{16}=&\frac{(a+b)^2}{2(a-b)}
\end{align*}

\begin{align*}
	a_{17}=&\frac{a^2-b^2}{2(a+3b)},     b_{17}= \frac{a^2-b^2}{2(3a+b)}\\
	a_{18}=&\frac{a^2-b^2}{2(a-3b)},     b_{18}= \frac{a^2-b^2}{2(3a-b)}\\
	a_{20}=&\frac{a^2-b^2}{a},     b_{20}=\frac{a^2-b^2}{b}\\
	a_{32}=& \frac {a \left( a^2-b^2 \right)   \left( 3\,{a}^
			{2}+5\,{b}^{2} \right) }{2(3\,{a}^{4}+2\,{a}^{2}{b}^{2}+3\,{b}^{4})}\\
   b_{32}=& \frac {b \left( a^2-b^2 \right)   \left( 3\,{a}^
			{2}+5\,{b}^{2} \right) }{2(3\,{a}^{4}+2\,{a}^{2}{b}^{2}+3\,{b}^{4})}\\
	a_{39}=&\frac { \left( {a}^{2}-{b}^{2} \right) a}{2( {a}^{2}+3\,{b}^{2})},
	b_{39}=\frac{ \left( {a}^{2}-{b}^{2} \right) b}{2(3 \,{a}^{2}+\,{b}^{2})}\\
	a_{61}=& \frac {    \left( a^2-b^2\right)  \left( 3\,a-b
			\right) }{2( 3a^{2}+2\,ab+3\,{b}^{2})}\\
	b_{61}=& \frac { \left( a^2-b^2 \right)  \left( a-3\,b \right)    }{2(3\,{a}^{2}+2\,ab+3\,{b}^{2})}\\
	a_{62}=&\,{\frac {  \left( a^2-b^2 \right)  \left( 3\,a+b
				\right) }{2(3\,{a}^{2}-2\,ab+3\,{b}^{2})}}\\
	b_{62}=&{\frac {  \left( a^2-b^2 \right)  \left( a+3b
					\right) }{2(3\,{a}^{2}-2\,ab+3\,{b}^{2})}}\\
				a_{69}=&{\frac { \left( a^2-b^2 \right)    a}{{a}^{2}+{b}^{2}}},\;\;
				b_{69}=\frac { \left( a^2-b^2 \right)    b}{{a}^{2}+{b}^{2}}\\
		a_{76}=&  \frac { \left( a^2-b^2 \right)    a}{{a}^{2}+3{b}^{2}},\;\; b_{76}= \frac{ \left( a^2-b^2 \right)    b}{3{a}^{2}+{b}^{2}}
\end{align*}
\begin{align*}
		a_{83}=&  \frac { \left( a^2-b^2 \right)    a}{5{a}^{2}+3{b}^{2}},b_{83}= \frac{ \left( a^2-b^2 \right)    b}{3{a}^{2}+5{b}^{2}}\\
		a_{98}=& \frac{a^2+b^2}{2a}, 	b_{98}= \frac{a^2+b^2}{2b}\\
		a_{99}=&a,\;\;
		b_{99}=b\\
a_{114}=& \frac{a^2+b^2}{4a}, 	b_{114}= \frac{a^2+b^2}{4b}\\
a_{115}=& \frac{a }{2}, 	\;\; b_{115}= \frac{b}{2}\\
				%
a_{140}=& \frac{a^2-b^2}{16a}, 	b_{140}= \frac{a^2-b^2}{16b}\\
a_{141}=&\frac{(a^2-b^2)a}{4(a^2+b^2)},
b_{141}= \frac{(a^2-b^2)b}{4(a^2+b^2)}\\
a_{147}=&\frac{a^2+b^2}{a},
					b_{147}= \frac{a^2+b^2}{b}\\
					a_{148}=&2{a},
					b_{148}=2b\\
		a_{182}=&\frac{(a^2-b^2)^2}{8a(a^2+b^2)},\;\;
					b_{182}= \frac{(a^2-b^2)^2}{8b(a^2+b^2)}\\
					a_{187}=& \frac{a(a^2+3b^2)}{2(a^2-b^2)},
						b_{187}=  \frac{b(3a^2+b^2)}{2(a^2-b^2)}\\
						a_{190}=& a,\;\; b_{190}=b\\
		a_{193}=&\frac{2(a^2-b^2)a}{a^2+b^2},\;
		b_{193}=\frac{2(a^2-b^2)b}{a^2+b^2}\\
		a_{194}=&\frac{2(a^2-b^2)a}{a^2+3b^2},
		b_{194}=\frac{2(a^2-b^2)b}{3a^2+b^2}				
\end{align*}

\subsection{Incircle}

\subsection{Circumcircle}

\subsection{Dual}

\subsection{Excentral}

==> overflow.tex <==



\begin{table}
\begin{minipage}{2.0in}
\begin{tabular}{|c|c|c|c|}
\hline
$X_k$ & $\alpha$ & $\beta$ & $\gamma$ \\
\hline
$X_1$ &$1$ & $0$ & $0$ \\
$X_2$ & $0$ & $1$ & $0$  \\
$X_3$ & $0$ & $0$ & $1$  \\
$X_4$ & $0$ & $3$ & $-2$ \\
$X_5$ & $0$ & $\frac{3}{2}$ & $-\frac{1}{2}$ \\
$X_7$ & $\frac{2\rho+4}{\rho+4}$ & $\frac{3\rho}{\rho+4}$ & $\frac{-4\rho}{\rho+4}$  \\
$X_8$ & $-2$ & $3$ & $0$ \\
$X_9$ & $\frac{-\rho-2}{\rho+4}$ & $\frac{6}{\rho+4}$ & $\frac{2\rho}{\rho+4}$\\
$X_{10}$ & $-\frac{1}{2}$ & $\frac{3}{2}$ & $0$  \\
$X_{11}$ & $\frac{1}{1-2\rho}$ & $\frac{-3\rho}{1-2\rho}$ &  $\frac{\rho}{1-2\rho}$  \\
$X_{12}$ & $\frac{1}{1+2\rho}$ & $\frac{3\rho}{1+2\rho}$ &  $\frac{-\rho}{1+2\rho}$  \\
$X_{20}$ & $0$ & $-3$ & $4$ \\
$X_{21}$ & $0$ & $\frac{3}{2\rho+3}$ & $\frac{2\rho}{2\rho+3}$  \\
$X_{35}$ & $\frac{1}{2\rho+1}$ &  $0$ & $\frac{2\rho}{2\rho+1}$ \\
$X_{36}$ & $\frac{1}{1-2\rho}$ & $0$ & $\frac{-2\rho}{1-2\rho}$  \\
$X_{40}$ & $-1$ & $0$ & $2$ \\
$X_{46}$ & $\frac{1+\rho}{1-\rho}$ & $0$ & $\frac{-2\rho}{1-\rho}$ \\
$X_{55}$ & $\frac{1}{1+\rho}$ & $0$ & $\frac{\rho}{1+\rho}$  \\
$X_{56}$ & $\frac{1}{1-\rho}$ & $0$ & $\frac{-\rho}{1-\rho}$ \\
$X_{57}$ & $\frac{2+\rho}{2-\rho}$ & $0$ & $\frac{-2\rho}{2-\rho}$  \\
$X_{63}$ & $\frac{-\rho-2}{\rho+1}$ & $\frac{3}{\rho+1}$ &  $\frac{2\rho}{\rho+1}$\\
$X_{65}$ & $\rho+1$ & $0$ & $-\rho$ \\ 
$X_{72}$ & $-\rho-2$ & $3$ & $\rho$ \\
$X_{78}$ & $\frac{\rho+2}{\rho-1}$ & $\frac{-3}{\rho-1}$ & $0$ \\ 
$X_{79}$ & 1 & $\frac{6\rho}{2\rho+3}$ & $\frac{-6\rho}{2\rho+3}$ \\ 
$X_{80}$ & $\frac{2\rho+1}{1-2\rho}$ & $\frac{-6\rho}{1-2\rho}$ &  $\frac{2\rho}{1-2\rho}$ \\
$X_{84}$ & $\frac{-\rho-2}{\rho}$ & $\frac{6}{\rho}$ & $\frac{2\rho-4}{\rho}$ \\ 
$X_{90}$ & $\frac{-(\rho+1)^2}{\rho^2+2\rho-1}$ & $\frac{6\rho}{\rho^2+2\rho-1}$ & $\frac{2\rho(\rho-1)}{\rho^2+2\rho-1}$\\ 
$X_{100}$ & $\frac{2}{2\rho-1}$ & $\frac{-3}{2\rho-1}$ & $\frac{2\rho}{2\rho-1}$ \\
$X_{104}$ & $\frac{-2}{2\rho-1}$ & $\frac{3}{2\rho-1}$ & $\frac{2\rho-2}{2\rho-1}$ \\ 
$X_{119}$ & $\frac{1}{2\rho-1}$ & $\frac{3\rho-3}{2\rho-1}$ & $\frac{-\rho+1}{2\rho-1}$ \\
$X_{140}$ & $0$ & $\frac{3}{4}$ & $\frac{1}{4}$  \\
$X_{142}$ & $\frac{\rho+2}{2\rho+8}$ & $\frac{3\rho+6}{2\rho+8}$ & $\frac{-2\rho}{2\rho+8}$ \\
$X_{144}$ & $\frac{-4\rho-8}{\rho+4}$ & $\frac{12-3\rho}{\rho+4}$ & $\frac{8\rho}{\rho+4}$\\
$X_{145}$ & $\frac{4}{7}$ & $\frac{3}{7}$ & $0$ \\
$X_{149}$ & $\frac{-4}{6\rho-3}$ &  $\frac{-6\rho+9}{6\rho-3}$ &  $\frac{12\rho-8}{6\rho-3}$ \\
$X_{153}$ & $\frac{4}{6\rho-3}$ & $\frac{-6\rho-3}{6\rho-3}$ & $\frac{12\rho-4}{6\rho-3}$ \\
$X_{165}$ & $-\frac{1}{3}$ & $0$ & $\frac{4}{3}$ \\
$X_{191}$ & $-1$ & $\frac{6}{2\rho+3}$ & $\frac{4\rho}{2\rho+3}$ \\
$X_{200}$ & $\frac{\rho+4}{\rho-2}$ & $\frac{-6}{\rho-2}$ & $0$ \\
\hline
\end{tabular}
\end{minipage}
